Connections between Mean-Field Game and Social Welfare Optimization

This paper studies the connection between a class of mean-field games and a social welfare optimization problem. We consider a mean-field game in function spaces with a large population of agents, and each agent seeks to minimize an individual cost function. The cost functions of different agents are coupled through a mean-field term that depends on the mean of the population states. We show that although the mean-field game is not a potential game, under some mild condition the $\epsilon$-Nash equilibrium of the mean-field game coincides with the optimal solution to a social welfare optimization problem, and this is true even when the individual cost functions are non-convex. The connection enables us to evaluate and promote the efficiency of the mean-field equilibrium. In addition, it also leads to several important implications on the existence, uniqueness, and computation of the mean-field equilibrium. Numerical results are presented to validate the solution, and examples are provided to show the applicability of the proposed approach.

==> Simulation.tex <==
\section{Demand Response Applications}
In this section, we apply the proposed approach to two applications: the charging of EV fleet, and the coordination of a group of  TCLs. Realistic simulation results are presented to demonstrate the effectiveness of the proposed approach.


\subsection{EV Fleet Charging}
In this example, a coordinator purchases energy from the wholesale energy market, and determines a price vector to efficiently allocate energy to a group of self-interested EVs over a finite discrete-time horizon. The EVs randomly arrive at and depart from the charging lot, and the vehicle should be fully charged before it departs. In this scenario, we assume that each random variable for different vehicles (including the arrival time, departure time, initial state of charge (SOC), battery capacity and the maximum charging rate) is independently and identically distributed. Furthermore, we assume that the EV owner prefers to receive a flat charging profile during his stay. For instance, if a vehicle requests $6$ kWh energy over 30 minutes, he prefers to receive  $1$ kWh for every 5-minute period, i.e., $e_i=(1,1,1,1,1,1)$,  to receiving a charging profile that is concentrated in a few periods, i.e., $e_i=(0,3,0,3,0,0)$.    To capture the user preference, we define a valuation function that quadratically penalizes the deviations of its SOC from a reference SOC trajectory, which corresponds to a charging profile that splits the energy requests of each vehicle evenly between its arrival and departure. Aside from the valuation function, the vehicle is also charged a price per unit energy. The valuation function minus the payment is the utility function for each user, which can be modeled as (\ref{individualutiltiy}). The individual user chooses energy consumption schedule to maximize the individual utility function, while the coordinator tries to maximize the total utility of all users minus the energy procurement cost. In our example, the energy procurement cost $\phi_k(\cdot)$ is simply the wholesale energy price multiplied by the total energy. This problem can be modeled as (\ref{eq:socialwelfaremax}), with the battery dynamics of each vehicle as follows:
\begin{align}
\label{batterydynamics}
\begin{cases}
z_i(t_k)=z_i(t_{k-1})+\dfrac{1}{\bar{z}_i}e_i^k \nonumber \\
0\leq e_i^k \leq \bar{e}_i^k \nonumber \\
0\leq z_i(t_k)\leq 1,
\end{cases}
\end{align}
where $z_i(t_k)$ denotes SOC of the battery, $\bar{z}_i$ is the battery capacity, and $e_i^k$ is the assigned energy in the $k$th period. Note that if the vehicle is not on-site at time $k$, then $\bar{e}_i^k=0$.


We comment that we do not assume the coordinator knows the realization of the random variables, such as arrival time, departure time, initial SOC, etc. Instead, he only knows their probability distribution. We argue that for a large population of EVs, the probability distribution contains sufficient information for the coordinator to determine the optimal price. This is because of the following: based on the optimality conditions (\ref{eq:conditions1}), the optimal solution to the Stackelberg game (\ref{eq:socialwelfaremax}) only depends on the aggregated energy response $\sum_{i=1}^Kh_i^k(p_c)$. The aggregated energy response is stochastic as its dependence on the random variables. However, for a large number of EVs, the variance of $\sum_{i=1}^Kh_i^k(p_c)$ is typically small due to the law of large numbers. Therefore, if we simulate the EV fleet and determine the unit price based on the aggregated energy response of the simulated fleet, then the derived price can be applied to the real EV fleet to induce an aggregated energy response that is close to the response of the simulated EV fleet. This indicates that the unit price derived based on simulated EVs is close to optimal for the real EV fleet.


In the simulation, we consider the 5-minute control period with a planning horizon of 6 hours.  Two realizations of the EV fleet data (each realization has 1000 EVs) are generated with the following random variables uniformly drawn from proper ranges: the arrival times of each vehicle (over 6 hours), the length of stay for each vehicle (between 2 hours and 4 hours), the battery capacity of the EV (between $15$ kWh and $20$ kWh) , the maximum charging rate for the fleet (between $6$ kW and $8$ kW), the initial SOC for the EV (between $0\%$ and $20\%$), and the parameters $\beta_i^k$ for individual utilities. We refer to these two sets of data as the simulated EV fleet and the real EV fleet, respectively. Based on preceding discussions, the optimal price is derived with the simulated EV fleet and then applied to the real EV fleet for verification. To obtain a close-to $100\%$ SOC at the end, the coefficient $\beta_i^k$ at departure is set to be significantly smaller than at other steps (note that $\beta_i^k<0$). In addition, we assume that the power capacity limit is $3.5$ MW, which corresponds to a 5 minute energy bound $D=3.5$ MWh$/12=291$ kWh. The cost function $\phi_k$ is assumed to be linear: the cost function $\phi_k(\cdot)$ is simply the wholesale energy price multiplied by the total energy consumption. The wholesale price data is derived from PJM's energy market \cite{PJMLMP}. In our paper, we refer to it as the base price, which corresponds to $p_w$.


The simulation uses the wholesale energy price data between $11:00$ AM and $17:00$ PM. We randomly select a vehicle with its reference SOC trajectory and the optimal SOC trajectory shown in Figure \ref{PEVstate}. This vehicle arrives at $11:55$AM with an initial SOC of $17\%$, and departs at $15:45$ PM. The optimal SOC trajectory is close to the reference, and the vehicle gets fully charged before departure. The optimal price and the base price trajectory are shown in Figure \ref{PEVprice}. Under the optimal price, the aggregated energy response for the simulated EV fleet and the real EV fleet is shown in Figure \ref{PEVenergy}. These two figures indicate that the derived solution is the optimal solution for the simulated EV fleet, as it satisfies the optimality conditions (\ref{eq:conditions1}): when the clearing price (coordinator's control) equals the base price, the aggregate energy of the simulated EV fleet is less than the total energy budget, and when the clearing price is greater than the base price, the total energy of the simulated EV fleet equals the energy budget. In addition, it is clear that the aggregated energy of the real EV fleet is very close to that of the simulated fleet, indicating that the derived price is close to optimal for the real fleet. 


\begin{figure}[t]%
\centering
\includegraphics[width = 0.8\linewidth]{figures/EV1}
\caption{The SOC trajectory and the reference between 11:00 AM and 5:00 PM.}
\label{PEVstate}
\end{figure}


\begin{figure}[t]%
\centering
\includegraphics[width = 0.8\linewidth]{figures/EV3}
\caption{The coordinator's control (clearing price) and the base price between 11:00 AM and 5:00 PM}
\label{PEVprice}
\end{figure}



\begin{figure}[t]%
\centering
\includegraphics[width = 0.85\linewidth]{figures/EV2}
\caption{The simulated total energy consumption, real energy consumption, and the total energy budget.}
\label{PEVenergy}
\end{figure}





\subsection{Coordination of Thermostatically Controlled Loads}
Similar to the EV example, we consider a coordinator who purchases energy from the wholesale energy market and allocates energy to a group of TCLs via pricing over a finite discrete-time horizon. Each user has a desired temperature and a valuation function that quadratically penalizes the deviations from desired temperature. Aside from valuation function, the user is also charged a price per unit energy. The valuation function minus the payment is the utility function for each user, which can be modeled as (\ref{individualutiltiy}).  We assume that the load parameters and individual utilities are known to the coordinator.  The individual user tries to maximize the individual utility function, while the coordinator wishes to maximize the total utility of all users minus the energy procurement cost. The energy procurement cost $\phi_k(\cdot)$ is the wholesale energy price multiplied by the total energy. This problem can be modeled as (\ref{eq:socialwelfaremax}), with the linear discrete-time system dynamics presented below.  




\subsubsection{Dynamic of TCLs}
The thermal dynamics of TCL are typically characterized by the continuous time Equivalent Thermal Parameter (ETP) model \cite{sonderegger1978dynamic}. The most widely used model in the literature is the first-order ETP model 
\cite{koch2011modeling}, \cite{callaway2009tapping}, \cite{sonderegger1978dynamic},  \cite{mathieu2013state},  which can be summarized as follows:
\begin{equation}
\label{eq:inddynamics}
\dot{z}_{i}(t)=\tilde{A}_{i}z_{i}(t)+\tilde{B}_{on}^{i} (\tilde{B}_{off}^i),
\end{equation}
where $z_i(t)$ denotes the room temperature, $\tilde{A}_i$ is a constant, and $\tilde{B}_{on}^i$ and $\tilde{B}_{off}^i$ are time-varying due to the outside environment disturbances. 

Now we show that the continuous time model (\ref{eq:inddynamics}) can be transformed to the discrete-time model (\ref{eq:discretedynamics}) under the following control policy: during each period (e.g., 5 minutes), the system is on from $t_{k-1}$ to $T_{1}$ (to be determined), off from $T_{1}$ to $T_{2}$, and on from $T_{2}$ to $t_{k}$, where $T_1$ and $T_2$ satisfy the following:
\begin{align}
\begin{cases}
T_1=\alpha T+\dfrac{1}{\tilde{A}_i}\text{ln}\dfrac{e^{(1-\alpha)\tilde{A}_iT}-1}{1-\alpha}-\dfrac{1}{\tilde{A}_i}\text{ln}(e^{\tilde{A}_iT}-1)\\
T_2=T+\dfrac{1}{\tilde{A}_i}\text{ln}\dfrac{e^{(1-\alpha)\tilde{A}_iT}-1}{1-\alpha}-\dfrac{1}{\tilde{A}_i}\text{ln}(e^{\tilde{A}_iT}-1)
\end{cases}
\label{eq:controlstrategy}
\end{align}
where $\alpha$ is the portion of time the system is on during one control period. It can be verified that the proposed control policy results in a linear discrete-time dynamic system (\ref{eq:discretedynamics}), where the parameters satisfy the following: 
\begin{align}
\begin{cases}
A_i=e^{\tilde{A}_iT}\\
B_i^k=\dfrac{(\tilde{B}_{on}^i-\tilde{B}_{off}^i)(e^{\tilde{A}_iT}-1)}{\bar{e}_i^k\tilde{A}_i} \\
C_i^k=\dfrac{\tilde{B}_{off}^i(e^{\tilde{A}_iT}-1)}{\tilde{A}_i}
\end{cases}
\label{eq:modelparameters}
\end{align}
Note that in the above equations, $A_i>0$, and $B_i^kB_i^j>0$, which satisfies our assumption in Section II-A.


\subsubsection{Simulation Results}
In the simulation, we generate 1000 sets of building parameters. The thermal capacity, the thermal resistance and the rated power of each load are generated based on a uniform distribution. We assume the average power of the TCL loads is 5 kW, and the feeder power capacity is 2.5 MW, and the parameters of the agent utility function are generated based on a uniform distribution. 

The ETP model parameters depend on the air temperature \cite{sonderegger1978dynamic}. Here we use the air temperature data for Columbus, OH, obtained from \cite{weatherdata}. Similar to example 1, we consider a linear cost function $\phi_k$ and refer to the wholesale energy price as the base price.






\begin{figure}[bt]%
\centering
\includegraphics[width = 0.8\linewidth]{figures/TCL1}
\caption{The state trajectory of a randomly selected TCL between 11:00 AM and 2:00 PM.}
\label{fig1}
\end{figure}


\begin{figure}[bt]%
\centering
\includegraphics[width = 0.8\linewidth]{figures/TCL3}
\caption{The aggregated resource trajectory and the resource constraint between 11:00 AM and 2:00 PM.}
\label{fig2}
\end{figure}

\begin{figure}[bt]%
\centering
\includegraphics[width = 0.8\linewidth]{figures/TCL2}
\caption{The coordinator's control (clearing price) and the base price between 11:00 AM and 2:00 PM. The clearing price is higher than the base price during power congestion.}
\label{fig3}
\end{figure}




Simulations are run for the TCLs using the temperature record and energy price record between $11:00$ AM and $14:00$ PM. A TCL is randomly selected, whose state trajectory is shown in Figure \ref{fig1}. Simulation result shows that the state constraint is always respected. The total energy trajectory is shown in Figure \
\ref{fig2}. Since the feeder capacity limit is $2.5$ MW, the total energy constraint during each 5-minute period is $2.5$ MWh$/12=208.3$ kWh. The simulation result shows that this energy constraint is always respected throughout the entire horizon. In addition, the coordinator's control (referred to as the clearing price) and the base price are shown in Figure~\ref{fig3}. We observe that when there is no power congestion, the  clearing price is equal to the base price. When power congestion occurs, the clearing price is higher than the base price, and the energy during the congestion period is exactly equal to the energy cap (can be verified in Figure~\ref{fig2}). This is consistent with the sufficient conditions for the optimal price (\ref{eq:conditions1}).




